Communication-Efficient Distributed Deep Learning: A Comprehensive Survey

Distributed deep learning (DL) has become prevalent in recent years to reduce training time by leveraging multiple computing devices (e.g., GPUs/TPUs) due to larger models and datasets. However, system scalability is limited by communication becoming the performance bottleneck. Addressing this communication issue has become a prominent research topic. In this paper, we provide a comprehensive survey of the communication-efficient distributed training algorithms, focusing on both system-level and algorithmic-level optimizations. We first propose a taxonomy of data-parallel distributed training algorithms that incorporates four primary dimensions: communication synchronization, system architectures, compression techniques, and parallelism of communication and computing tasks. We then investigate state-of-the-art studies that address problems in these four dimensions. We also compare the convergence rates of different algorithms to understand their convergence speed. Additionally, we conduct extensive experiments to empirically compare the convergence performance of various mainstream distributed training algorithms. Based on our system-level communication cost analysis, theoretical and experimental convergence speed comparison, we provide readers with an understanding of which algorithms are more efficient under specific distributed environments. Our research also extrapolates potential directions for further optimizations.

==> related.tex <==
\section{related work}\label{sec:related}

Two surveys ~\citep{Peteiro2013,8005992} provide a general introduction of distributed machine learning algorithms for dealing with big data. Xing et al. ~\citep{XING2016179} discuss distributed machine learning on big data, mainly covering different synchronization schemes, scheduling, and balancing workloads and communication typologies. Ben-Nun et al. ~\citep{10.1145/3320060} provide a review of distributed deep learning, mostly focusing on DNN operators and some main approaches for parallelism for both training and inference. Guo ~\citep{DBLP:abs-1808-04752} gives a thorough review of different quantized neural networks, which offers some insights to quantized SGD optimization. Zhang et al. ~\citep{8644613} provide a quick survey on large-scale distributed deep learning systems, which concisely introduces parallelisms, parameter server architectures, synchronization schemes, related applications, and platforms.

Different from the two surveys ~\citep{10.1145/3320060,8644613} that are mostly related to ours, we mainly focus on communication-efficient distributed deep learning training. The two surveys ~\citep{10.1145/3320060,8644613} lack of detailed discussions on communication compression techniques, which are introduced explicitly in this survey. Moreover, we give a quick review of some auxiliary technologies and also provide the convergence bound comparisons.

==> taxonomy_old.tex <==
\section{Taxonomy of Distributed SGD}\label{sec:problemformulation}

The mathematical formulation of DL can be defined as the following optimization problem:
\begin{equation}\label{eq:single_dl}
    \min \limits_{\mathbf{x}\in \mathbb{R}^N }f_{s}(\mathbf{x}):=\mathbb{E}_{\xi_i \sim \mathcal{D}} F(\mathbf{x};\xi_i),
\end{equation}
where the random variable $\xi_i$ has a probability distribution $\mathcal{D}$, referring to data samples from a dataset, $\mathbf{x}$ represents all the parameters of the model, $N$ is the number of parameters, and $f_{s}:\mathbb{R}^N \to \mathbb{R}$ is the objective function. 

Gradient-based optimization algorithms are the most widely used in solving the above optimization problem in DL. Due to high computation complexity of second-order gradient descent methods with DNNs, the first-order gradient descent methods, especially the stochastic gradient descent (SGD) with mini-batch\footnote{To simplify, throughout this paper, we use SGD to denote the training algorithm of SGD with mini-batch which includes the cases of one sample and more than one samples in each training iteration.} and it variants, are commonly used in DL. The update rule of \textbf{single-device} SGD has the following form. 
\begin{equation}
    G_{t}(\mathbf{x}_{t}) = {\nabla}F_{t}(\mathbf{x}_{t};\xi_{t})
\end{equation}
\begin{equation}\label{eq:sgd}
    \mathbf{x}_{t+1} = \mathbf{x}_{t} - {\gamma}G_{t}(\mathbf{x}_{t}),
\end{equation}
where $\mathbf{x}_t \in \mathbb{R}^N$ is the $N$-dimensional model parameter at iteration $t$, $\xi_{t}$ is a randomly sampled mini-batch of data, and $\gamma$ is the learning rate (or step size). SGD is an iterative algorithm and has been proved that it can solve \eqref{eq:single_dl} under the assumptions that $f_s(\mathbf{x})$ is non-convex and is with L-Lipschitzian gradients ~\citep{Bottou2016OptimizationMF}. The iterative process generally contains several steps: 1) It samples a mini-batch of \textbf{data} (i.e., $\xi_{t}$). 2) It performs the \textbf{feed-forward} computations to calculate the loss value (i.e., $F_{t}(\mathbf{x}_{t};\xi_{t})$) of the objective function. 3) It performs the \textbf{backward propagation} to calculate the gradients (i.e., ${\nabla}F_{t}(\mathbf{x}_{t};\xi_{t})$) with respect to the model parameters. 4) Finally, it \textbf{updates} the model parameters by Eq. \eqref{eq:sgd}. 

% Because training a large DNN time-consuming, it becomes common to exploit multiple processors to accelerate the training process using distributed training techniques.

Distributed training modifies the above four single-device SGD procedures into distributed versions. We firstly describe the procedures of the basic distributed training algorithm, i.e. \textbf{bulk synchronous parallel SGD} (BSP-SGD) ~\citep{BSP7917379181}, and then elucidate how other algorithms different from it.
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/figure_timeline2.pdf}
	\vspace{-10pt}
	\caption{Comparison of training with single device and multiple devices under different communication synchronization with the PS architecture.}
	\label{fig:timeline}
\end{figure}

In BSP, each worker (say worker $i$, and $i=1,2,...,n$) pulls down the whole global model from the Parameter Server (PS), and then loads different data (i.e., $\xi_{i,t}$) and independently calculates the gradients (${\nabla}F(\mathbf{x}_t;\xi_{i,t})$) at the same time. Before updating the model, the gradients are aggregated on the PS and all workers are synchronized by the barrier before beginning the next iteration. At last, the PS average all received local gradients to update the global model. The timeline of BSP is shown in Fig. \ref{fig:timeline}. 

The update rule of BSP-SGD can be formulated as: 
% \begin{equation}\label{eq:ssgd_gra}
%     G_{i,t}(\mathbf{x}_{t}) = {\nabla}F_{i,t}(\mathbf{x}_{t};\xi_{i,t})
% \end{equation}
% \begin{equation}\label{eq:ssgd_upd}
%     \mathbf{x}_{t+1} = \mathbf{x}_{t} - {\gamma}\frac{1}{n}\sum_{i=1}^{n}G_{i,t}(\mathbf{x}_{t}),
% \end{equation}
\begin{align}
    G_{i,t}(\mathbf{x}_{t}) & = {\nabla}F_{i,t}(\mathbf{x}_{t};\xi_{i,t}) \label{eq:ssgd_gra} \\  
    \mathbf{x}_{t+1} & = \mathbf{x}_{t} - {\gamma}\frac{1}{n}\sum_{i=1}^{n}G_{i,t}(\mathbf{x}_{t}), \label{eq:ssgd_upd}
\end{align}

where $G_{i,t}(\mathbf{x}_{t})$ represents the gradient of $F_{i,t}(\mathbf{x}_{t})$ of worker $i$ at iteration $t$. 

% In the above scheme, there exist three key factors affecting the communication cost:
% \begin{enumerate}
% \item Communication synchronization and frequency of the $n$ participating workers;
% \item The aggregation algorithm of $n$ vectors in distributed memory;
% \item The communication traffic related to the dimension of the model (i.e., $N$).
% \end{enumerate}

Algorithms that improve BSP can be classified into four orthogonal dimensions:
\begin{enumerate}
    \item \textbf{Flexible synchronization} considers relaxing the strict synchronization of BSP to reduce the impact of synchronization and the number of communications in the same period.
    \item \textbf{Different system architectures} aim to change the communication topology to avoid the communication congestion of the PS and workers. 
    \item \textbf{Compression techniques} intend to compress the communication data to reduce communication traffic and thus reduce the communication time.
    \item \textbf{The parallelism of communication and computing} tries to hide the communication time to achieve shorter iteration time.
\end{enumerate}
According to this taxonomy, an overview of the distributed deep learning is shown in Fig. \ref{fig:overview}. And readers can find a comparison in Table~\ref{tab:Taxonomy_DisSGD} to get an overall understanding. We give a simple discussion of these dimensions in the following subsections.

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{figures/figure_researchsummary.pdf}
	\vspace{-10pt}
	\caption{Overview of distributed deep learning.}
	\label{fig:overview}
\end{figure*}


% As discussed in Section \ref{sec:intro}, the original BSP-SGD could easily suffer from the communication bottleneck due to the high communication synchronization frequency and the high model/gradient aggregation cost. Communication-efficient distributed training algorithms aim to address the communication problems while providing convergence guarantees, which can be summarized to four dimensions, including communication synchronization, system architectures, compression techniques, and parallelism of communication and computing, as shown in Table \ref{tab:Taxonomy_DisSGD}. 

\begin{table}[t]
  \centering
  \fontsize{7}{7}\selectfont
  \begin{threeparttable}
  \caption{Taxonomy of Distributed SGD}
  \label{tab:Taxonomy_DisSGD}
    \begin{tabular}{cc}
    \toprule
    Dimension & Method \cr
    \midrule
    %\multicolumn{2}{c}{\bf Model Consistency}\cr
    \multirow{2}{*}{\bf xxxx } & Model Parallelism \cr
    & Data Parallelism \cr
    \hline
    \multirow{4}{*}{\bf Communication Synchronization} & Synchronous \cr
    & Stale-Synchronous \cr
    & Asynchronous \cr
    & Local SGD\cr
    \hline
    %\multicolumn{2}{c}{\bf Parameter Architecture and Communication}\cr
    \multirow{3}{*}{\bf System Architectures} & Parameter Server \cr
    & All-Reduce \cr
    & Gossip \cr
    \hline
    %\multicolumn{2}{c}{\bf Compression Techniques}\cr
    \multirow{3}{*}{\bf Compression Techniques} & Quantization \cr
    & Coding \cr
    & Sparsification \cr
    \hline    
    \multirow{2}{*}{\shortstack[c]{\bf Parallelism of\\\bf Communication and Computing}} & Pipelining \cr
     & Scheduling \cr
    % \cr    
    \bottomrule
    \end{tabular}
    \end{threeparttable}
\end{table}


\subsection{xxxxxxxxxx}

In terms of the parallelism schemes of distributed training, there exist two main types: data parallelism and model parallelism. 

% \subsubsection{Data Parallelism}
% The other main type of distributed training is data parallelism, as shown in Fig. \ref{fig:model_data_para}(b), in which the model parameters are replicated to all computing workers. In a single iteration, each computing worker processes different mini-batches of data to calculate the local gradient updates which are exchanged with the other workers before updating the model parameters. When using distributed multiple workers in data parallelism, the optimization problem of Eq. (\ref{eq:single_dl}) is changed into a new form:
\textbf{Data parallelism} is the mostly used type of distributed training, as shown in Fig. \ref{fig:model_data_para}(a), in which the model parameters are replicated to all computing workers. In a single iteration, each worker samples different mini-batches of data to calculate the local gradient or model updates and then exchanges them with the other workers. Then the aggregation and broadcast operations are executed to attain the new global model. When using distributed multiple workers in data parallelism, the optimization problem of Eq. (\ref{eq:single_dl}) is changed into a new form:

\begin{equation}\label{eq:data_para}
    f^*:= \min \limits_{\mathbf{x}\in \mathbb{R}^d } \left[ f(\mathbf{x}):=\frac{1}{n} \sum_{i=1}^n \underbrace{\mathbb{E}_{\xi_i \sim \mathcal{D}_i} 
    F_i(\mathbf{x};\xi_i)}_{=:f_i(\mathbf{x})}  \right]
\end{equation}
where $f_i:\mathbb{R}^d \to \mathbb{R}$ represents the objective function of worker $i$, and $n$ denotes the number of workers. This distributed optimization problem aims to minimize the mean of the objective functions at all workers.

% \subsubsection{Model Parallelism}
% Model parallelism splits model parameters to multiple computing workers ~\citep{dean2012large}. Every worker holds different parameters or layers of the model (i.e., a subset of $x$). There are two main types to split the model in model parallelism, which are shown in Fig. \ref{fig:model_para}(a) and Fig. \ref{fig:model_para}(b) respectively. Due to the high dependency between different neurons in the deep model, each worker should exchange its output results with the other workers before continuing the computation of the next layer. One main advantage of model parallelism is that training huge size models becomes possible since each worker can only hold a subset of the model, and thus the memory requirement is low. However, the model parallel methods have several key issues, such as the unbalance parameter sizes and the high computing dependency in different layers of the deep model ~\citep{dean2012large}. It is non-trivial and even NP-complete ~\citep{3154842} to split the learning model into suitable parts and assign them appropriately to different computing nodes. Furthermore, one needs to design an elaborate algorithm to guarantee the robustness of model parallelism, which is difficult due to computing dependency. Because of these issues, it is not trivial to accelerate the training with model parallelism ~\citep{Mirhoseini2017}.

\textbf{Model parallelism} splits model parameters to multiple computing workers ~\citep{dean2012large}. Every worker holds different parameters or layers of the model (i.e., a subset of $x$). There are two main types to split the model in model parallelism, which are shown in Fig. \ref{fig:model_data_para}(b). Due to the high dependency between different neurons in the deep model, each worker should exchange its output results with the other workers before continuing the computation of the next layer. One main advantage of model parallelism is that training huge size models becomes possible since each worker can only hold a subset of the model, and thus the memory requirement is low. However, the model parallel methods have several key issues, such as the unbalance parameter sizes and the high computing dependency in different layers of the deep model ~\citep{dean2012large}. It is non-trivial and even NP-complete ~\citep{3154842} to split the learning model into suitable parts and assign them appropriately to different computing nodes. Furthermore, one needs to design an elaborate algorithm to guarantee the robustness of model parallelism, which is difficult due to computing dependency. Because of these issues, it is not trivial to accelerate the training with model parallelism ~\citep{Mirhoseini2017}.


\begin{figure*}[t]
	\centering
	\subfigure[Data parallelism.]
	{
	\includegraphics[width=0.45\linewidth]{figures/figure_data_para.pdf}
	}
    \subfigure[Model parallelism.]
	{
	\includegraphics[width=0.45\linewidth]{figures/figure_model_para2.pdf}
	}
	\caption{Model parallelism v.s. Data parallelism. Each dotted color box represents the parameters assigned to a worker. The thick lines represent the data communication between different workers.}
	\label{fig:model_data_para}
\end{figure*}


% \begin{figure*}[t]
% 	\centering
%     \subfigure[Type 1.]
% 	{
% 	\includegraphics[width=0.45\linewidth]{figures/figure_model_para.pdf}
% 	}
% 	\subfigure[Type 2.]
% 	{
% 	\includegraphics[width=0.45\linewidth]{figures/figure_model_para2.pdf}
% 	}
% 	\caption{Model parallelism. Each color represents one part of the model that is assigned to a worker. The thick lines represent the data communication between different workers.}
% 	\label{fig:model_para}
% \end{figure*}

% \begin{figure}[!h]
% 	\centering
% 	\includegraphics[width=0.98\linewidth]{figures/figure_data_para.pdf}
% 	\vspace{-10pt}
% 	\caption{Data parallelism.}
% 	\label{fig:data_para}
% \end{figure}

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.45\linewidth]{figures/figure_data_para.pdf}
% 	\vspace{-10pt}
% 	\caption{Data parallelism.}
% 	\label{fig:data_para}
% \end{figure}







% With the help of Fig. \ref{fig:timeline}, we summarize the procedure of BSP with PS architecture as follows:
% \begin{enumerate}
% \item \textit{Pulling the updates}. Each worker attains the newest model from parameter servers (CM1 in Fig. \ref{fig:timeline}).
% \item \textit{Computation}. Each worker samples the data independently and feeds it into its local model to calculate the gradients (CP in Fig. \ref{fig:timeline}). Based on different optimization algorithms, how to use the gradients to get the parameter updates is different. For SGD, the updates are gradients itself.
% \item \textit{Pushing the updates}. Communicates the parameter updates to servers (CM2 in Fig. \ref{fig:timeline}).
% \item \textit{Update Model}. When all workers complete communication (Synchronous Barrier), parameter servers do the model update.
% \end{enumerate}

% Then we will concisely illustrate different methods from these three dimensions, and indicate where they are different from BSP-SGD with the PS architecture.

\subsection{Communication synchronization}


% There are some important issues that the multi-devices bring:

%First, the models are distributed across all the computing nodes, and then with the different data they sample, the different updates will come. Therefore, one of the nodes may hold a different version of the model from others. Whether one should train the old local model or the newest global model is an important question. Keeping the local model same with the global model will take a cost of time-consuming communication. But to let the local model train itself in a long time will make the future training performance decreases severely. Based on this question, people developed different techniques to alleviate it, like to find a balance between the full synchronization and non-synchronization ~\citep{SolvingtheStraggler} or to make use of algorithms of asynchronization  ~\citep{AsynDisOptimRandADMM,AsynDisADMM,AsynCoordD}.

% Second, in the data sampling phase, to decide which part of data that one of the devices should sample is an important question. For instance, if devices sample data following the non-i.i.d. distribution, to attain the same accuracy of single-device training is challengeable ~\citep{FLStrategy}. Usually, people are able to make the data sampling i.i.d., which is beneficial to the training. In some situations, however, the i.i.d. data sampling is impossible to attain, like Federated learning ~\citep{Federatedlearning}. 


% . Sometimes $f_i$ is $\mu$-strongly convex, but in most scenarios of immensely complicated tasks, $f_i$ is non-convex.
% When one exploits multi-devices to train a model, the training process is totally different. 

% Based on how many workers there are and how frequently each one works with others, data parallel methods can be split into four kinds of frameworks, synchronous, stale-synchronous, asynchronous, and local SGD. We will illustrate these methods in Section \ref{sec:async} in detail. The communication synchronization decides how frequently all local models are synchronized with others, which will influence not only the communication traffic but also the performance and convergence of model training. So there is a trade-off between the communication traffic and the convergence. Additionally, different synchronization schemes can be combined with different architectures. Here we introduce these four synchronization schemes under PS architecture due to its most extensive range of applications.

The \textbf{synchronization} in the data parallel distributed deep learning means that, before the next training round, the server must wait for all workers to finish the transmission of all parameters in the current iteration. The flexible synchronization will influence not only the communication traffic, but also the performance and convergence of model training. So there is a trade-off between the communication traffic and the convergence. Additionally, different synchronization schemes can be combined with different architectures. Here we introduce these four synchronization schemes under PS architecture due to its most extensive range of applications.


\subsubsection{Synchronous}
The classical algorithm of the synchronous framework is the mentioned BSP as shown in Fig. \ref{fig:timeline}, which generally requires the following steps: 1) Load the data; 2) Feed-forward computations; 3) Backward propagation computations; 4) Gradient aggregation with a barrier; and 5) Update the model with aggregated gradients. The synchronization of all workers could make the stragglers in the cluster extremely influence the overall system throughput. The full data aggregation of all workers also introduce very high communication cost, which severely limits the system scalability.

\subsubsection{Stale-Synchronous}
The stale-synchronous parallel (SSP) framework ~\citep{MoreEffDMLviaStaleSync} aims to alleviate the straggler problem without losing synchronization. As shown in Fig. \ref{fig:timeline}, it allows the faster workers to do more updates than the slower workers to reduce the waiting time of the faster workers.  However, to keep the model consistency to guarantee the convergence, there is a staleness bounded barrier, which limits the iteration gap between the fastest worker and the slowest worker. For a maximum staleness bound $s$, the update formula of worker $i$ at iteration $t+1$ is changed to
\begin{align}
    \mathbf{x}_{i,t+1} &=  \mathbf{x}_{0} - {\gamma}\sum_{k=1}^{t}\sum_{j=1}^{n}G_{j,k}(\mathbf{x}_{j,k})\notag \\ 
    &- {\gamma}\sum_{k=t-s}^{t}G_{i,k}(\mathbf{x}_{i,k}) - {\gamma}\sum_{(j,k)\in\mathcal{S}_{i,t+1}}G_{j,k}(\mathbf{x}_{j,k}), \label{eq:SSGSGD}
\end{align}
where $\mathcal{S}_{i,t+1}$ is some subset of the updates from other workers during period $\left[ t-s\right]$.

\subsubsection{Asynchronous}
Compared with the SSP framework, the asynchronous parallel (ASP) framework ~\citep{10.5555/2969442.2969545} completely eliminates the synchronization. As shown in Fig. \ref{fig:timeline}, each work transmits its gradients to the PS after it calculates the gradients. Then the PS updates the global model without waiting for the other workers. Note that ASP is not friendly to MPI collectives. The update formula of asynchronous SGD can be summarized as
\begin{equation}\label{eq:asyncsgd}
    \mathbf{x}_{t+1} =  \mathbf{x}_{t} - {\gamma}\sum_{i=1}^{n}G_{i,t-\tau_{i,k}}(\mathbf{x}_{i,t-\tau_{k,i}}),
\end{equation}
where the $\tau_{k,i}$ is the time delay between the moments when worker $i$ calculates the gradient at the current iteration. 

\subsubsection{Local SGD}
Another algorithm with strict synchronization but flexible communication frequency  is Local SGD~\citep{Sebastian2019}, which makes all workers run several or more iterations itself, and then averages all local models into the newest global model. There is a method named Model Average, which is very similar to Local SGD, locally running lots of iterations and does synchronization. The procedure of Local SGD can be formalized as
\begin{equation}\label{eq:localsgd}
    \mathbf{x}_{i, t+1} = \left \{
    \begin{array}{ll}
    \mathbf{x}_{i,t} - {\gamma}G_{i,t}(\mathbf{x}_{i,t}) ,& \text{if} \ t + 1 \not\in \mathcal{I}_T\\
    \mathbf{x}_{i,t} - {\gamma}\frac{1}{n}\sum_{i=1}^{n}G_{i,t}(\mathbf{x}_{i,t}), & \text{if} \ t + 1 \in \mathcal{I}_T
    \end{array}
    \right .
\end{equation}
where $\mathcal{I}_T$ represents the synchronization timestamps.

\subsection{System Architectures}
In terms of how to average the model parameters/gradients among distributed workers, we classify system architectures into three classes: Parameter Server (PS), All-Reduce, and Gossip.

% Here, we have two different dimensions of the topology of computing nodes. One is the communication topology, and the other is the model topology. The centralized communication topology means that the nodes communicate with others in a centralized way, and the decentralized communication topology in a decentralized way. And the model-centralized topology means there is always a global model kept, and vice versa.

%Here, the meaning of a centralized framework has two aspects, the logically centralized topology and the existence of a global model. Depending on whether there is logically centralized topology or not and whether there is a global model or not, 

\begin{figure*}[!h]
	\centering
    \subfigure[PS architecture.]
	{
	\includegraphics[width=0.25\linewidth]{figures/figure_PSarchitecture.pdf}
	}
	\subfigure[All-Reduce architecture.]
	{
	\includegraphics[width=0.3\linewidth]{figures/figure_MPIarchitecture.pdf}
	}
	\subfigure[Gossip architecture.]
	{
	\includegraphics[width=0.3\linewidth]{figures/figure_DECENTarchitecture.pdf}
	}
	\caption{Three different system architectures for model/gradient aggregation.}
	\label{fig:architectures}
\end{figure*}


\subsubsection{Parameter Server}
The Parameter Server (PS) architecture is shown in Fig. \ref{fig:architectures}(a). Servers are responsible for saving the newest global model, and collecting the updating information from the workers. Workers independently load the dataset, pull the newest global model from the server, and then compute the updates, which will be transmitted to the servers ~\citep{Smola2010}. In this architecture, the servers are the center of the communication topology, so the PS architecture is generally referred as the centralized framework, which is widely used in distributed training ~\citep{PSforDisML,ScalDMLwithPS,dean2012large,MoreEffDMLviaStaleSync,communicationDisMLwithPS,Ooi2015SD}. The main challenge of the PS architecture is the communication congestion in the server ~\citep{Zhang2015DLE296,HowToScaleDDL}, due to all workers communicating to the server. 

%In PS architecture, there is a global model kept, which continually communicates parameters with the local models. Note that the global model is not necessarily only stored in the servers, but can be also stored in the workers, depending on whether it is the parameter-server architecture or the all-reduce one. Or, in the gossip algorithms, there is no global model existing, which is replaced by the output of the consensus of models that all the workers would finally reach. In the later sections, we will illuminate this procedure more specifically under different manners of distribution and communication.

\subsubsection{All-Reduce}
To avoid the communication bottleneck in the PS, researchers prefer to use the All-Reduce architecture ~\citep{awan2017s,chu2017efficient,wang2019impact,goyal2017accurate,jia2018highly} to implement the gradient aggregation without central servers.

As shown in Fig. \ref{fig:architectures}(b), there is only one role, worker, in this method. All workers communicate without a central node. After the communication, they acquire all gradients of all workers and then update their local model, which is consistent with others. So, All-Reduce is a decentralized communication topology and a model-centralized topology since there is a consistent global model attained by synchronization. This makes there is no change in the updating Eq. \eqref{eq:ssgd_upd} using BSP-SGD. Note that this architecture is not suitable for asynchronous communication because the collective communication fashion of All-Reduce. And it is difficult to apply All-Reduce in the asynchronous part in SSP, but it is easy to apply it in the synchronous part in SSP.

% One of the disadvantages of All-Reduce is the lack of fault tolerance. Once one of the workers fails to work, the whole communication must be stopped and restart.

\subsubsection{Gossip}
The Gossip architecture is a kind of between-neighbors communication used to solve the distributed average problem ~\citep{gossip1,gossip2,gossip3,gossip4}. And many researchers exploit it to improve data parallel distributed SGD ~\citep{DisSubGradMultiOptim,AsynDisOptimRandADMM,OptimDisOptim,OptimNonsmoothDisOptim,DualApprochforOptim,MultiagentMirrorDescentDenct,CommEffDenctStoc,CanDecent,DecentTrainingoverDecentData,StocGradPush,CommCompforDecent}.

As shown in Fig. \ref{fig:architectures}(c), the gossip architecture here has either no parameter servers nor global model (represented by different colors of local models). Every worker communicates updates with their neighbors (also named peers). Workers exchange messages via those edges chosen in the current iteration (the blues ones in Fig. \ref{fig:architectures}(c)), which can be described in a communication graph. Communication with only neighbors means that workers do not need to communicate with everyone else. After one communication during training, the algorithm does not guarantee the consistency of parameters across all workers, but does guarantee it at the end of the algorithm. In other words, all local models are different during every iteration. Note that in asynchronous and SSP with the PS architecture, the local models are different, but the PS architecture keeps a global model, while the gossip architecture does not.


\subsection{Compression Techniques}
The compression methods consider compressing the gradients or model parameters that need to be transmitted to the workers or servers, to reduce the communication data. Most of the methods are lossy compression, which means that the original gradients or model parameters can not be fully recovered by the receiver. With less information gathered, the convergence could be sacrificed. It has been an active research direction to reduce the communication traffic with little impact on the convergence. Two main compression techniques, quantization and sparsification, are shown in Fig. \ref{fig:compression}. 
\begin{figure}[!ht]
	\centering
	\includegraphics[width=0.45\linewidth]{figures/figure_compression.pdf}
	\vspace{-10pt}
	\caption{Comparison of Quantization and Sparsification.}
	\label{fig:compression}
\end{figure}

\subsubsection{Quantization}
The quantization method is a kind of compression scheme that uses lower bits to represent the data which is originally represented by 32 bits on every dimension of the transmitted gradient. As shown in Fig. \ref{fig:compression}, the element in the quantized gradient is coded by fewer bits. Therefore, after the quantized communication, the gradients used to optimize the models are of low precision. Quantization of transmitted gradients is closely relevant to the deep learning with low precision. Deep learning with low precision is born in an environment where CPU and GPU need higher-speed calculating and lower memory for training DNNs. If the low precision of gradients can guarantee the convergence of training, the quantized communication is practicable. There have been already many researchers approaching the convergence of deep learning under the low-precision gradients ~\citep{ImproSpeedNN,DLwithlimited,ProbroundingNN,DorefaNet,Hubara2017}.

\subsubsection{Sparsification}
Sparsification methods aim to reduce the number of elements that are transmitted at each iteration. The key idea of sparsification is that in the update of SGD, only ``significant''  gradients are required to update the model parameter to guarantee the convergence of the training ~\citep{DGC}. As shown in Fig. \ref{fig:compression}, a large proportion of the coordinates of the gradient vector are zeroed-out such that the zero-valued elements are no need to transmit. Gradient sparsification is a more aggressive compression technique to reduce the communication traffic than quantization.

%The quantization methods can only achieve a maximum compression rate of x32. Because at least $1$ bit of every element in one gradient vector should be transmitted in quantization methods. If one reduce the number of elements that would be transmitted, the compression rate will be further increased. A series algorithms containing this ideology belong to sparsification methods, in which only a part of elements are chosen and then transimitted.


\subsection{Parallelism of Communication and Computing}
The layer-wise structure of deep models makes it possible to parallels the communication tasks and computing tasks. The parallelism of communication and computing mainly aims to optimize the order of computation and communication such that the communication cost can be minimized ~\citep{zhang2017poseidon,Shi2018MGWFBPED,hashemi2018tictac,harlap2018pipedream,peng2019generic,jayarajan2018priority,DBLP:journals/corr/abs-1810-08313,8884800}. For example, the pipelining technique of wait-free backward propagation (WFBP) ~\citep{zhang2017poseidon,awan2017s} and merged-gradient WFBP (MG-WFBP) ~\citep{Shi2018MGWFBPED} is widely used in BSP-SGD. It is also possible to combine the pipelining with gradient compression so that one can schedule the parallelism between compressed gradients' communications and computations on compression and backward propagation ~\citep{zheng2019communication,shi2020layer,shi2020communication,aritra2020discrepancy}.

In summary, the benefit of efficient communication algorithms could not be free. The communication-efficient algorithms generally exchange less information than the naive method while they may sacrifice the convergence performance (e.g., model accuracy). To better demonstrate the different influences by these methods, we summarize the comparison in Table \ref{tab:Influences_DisSGD}.

\begin{table*}[htbp]
%\centering
\fontsize{7}{7}\selectfont
\begin{center}
\caption{Influences of different combinations of architectures and synchronization schemes}
\label{tab:Influences_DisSGD}
%\addtolength{\tabcolsep}{-5pt}
\begin{threeparttable}        
\begin{tabular}{cccccc}
\hline
Architecture & Synchronization & Model consistency & Communication Frequency & Communication Congestion & Convergence \\ \hline\hline
\multirow{4}{*}{PS} & BSP & high & high & high & easy \\
 & SSP & normal & high & normal & normal \\  
 & ASP & low & high & low & difficult \\ 
 & Local SGD & normal & low & high & difficult \\   \hline
\multirow{4}{*}{All-Reduce} & BSP & high & high & low & easy \\  
 & SSP & - & - & - & - \\  
 & ASP & - & - & - & - \\ 
 & Local SGD & normal & low & low & difficult \\   \hline
\multirow{4}{*}{Gossip}  & BSP & low & high & low & normal \\ 
 & SSP & - & - & - & - \\ 
 & ASP & low & high & low & difficult \\ 
 & Local SGD & low & low & low & difficult \\ \hline

\end{tabular}
    \begin{tablenotes}    
        \footnotesize              
        \item Notes: Here the different levels only represent a relative description comparing with the other methods. The model consistency measures how local models are different from others, the communication frequency measures how frequently workers communicate with others, and communication congestion measures how heavy the traffic of the central node is.
      \end{tablenotes}          
\end{threeparttable}     
\end{center}
\end{table*}



% \begin{table*}[htbp]
% %\centering
% \fontsize{7}{7}\selectfont
% \begin{center}
% \caption{Influences of different combinations of architectures and synchronization schemes}
% \label{tab:Influences_DisSGD}
% %\addtolength{\tabcolsep}{-5pt}
% \begin{threeparttable}        
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Architecture & Synchronization & Model consistency & Communication Frequency & Communication Congestion & Convergence \\ \hline\hline
% \multirow{4}{*}{PS} & BSP & high & high & high & easy \\ \cline{2-6} 
%  & SSP & normal & high & normal & normal \\  \cline{2-6} 
%  & ASP & low & high & low & difficult \\  \cline{2-6} 
%  & Local SGD & normal & low & high & difficult \\   \hline
% \multirow{4}{*}{All-Reduce} & BSP & high & high & low & easy \\  \cline{2-6} 
%  & SSP & - & - & - & - \\  \cline{2-6} 
%  & ASP & - & - & - & - \\  \cline{2-6} 
%  & Local SGD & normal & low & low & difficult \\   \hline
% \multirow{4}{*}{Gossip}  & BSP & low & high & low & normal \\  \cline{2-6} 
%  & SSP & - & - & - & - \\  \cline{2-6} 
%  & ASP & low & high & low & difficult \\ \cline{2-6} 
%  & Local SGD & low & low & low & difficult \\ \hline

% \end{tabular}
%     \begin{tablenotes}    
%         \footnotesize              
%         \item Notes: Here the different levels only represent a relative description comparing with the other methods. The model consistency measures how local models are different from others, the communication frequency measures how frequently workers communicate with others, and communication congestion measures how heavy the traffic of the central node is.
%       \end{tablenotes}          
% \end{threeparttable}     
% \end{center}
% \end{table*}







